Multilingual Detection of Personal Employment Status on Twitter

Detecting disclosures of individuals' employment status on social media can provide valuable information to match job seekers with suitable vacancies, offer social protection, or measure labor market flows. However, identifying such personal disclosures is a challenging task due to their rarity in a sea of social media content and the variety of linguistic forms used to describe them. Here, we examine three Active Learning (AL) strategies in real-world settings of extreme class imbalance, and identify five types of disclosures about individuals' employment status (e.g. job loss) in three languages using BERT-based classification models. Our findings show that, even under extreme imbalance settings, a small number of AL iterations is sufficient to obtain large and significant gains in precision, recall, and diversity of results compared to a supervised baseline with the same number of labels. We also find that no AL strategy consistently outperforms the rest. Qualitative analysis suggests that AL helps focus the attention mechanism of BERT on core terms and adjust the boundaries of semantic expansion, highlighting the importance of interpretable models to provide greater control and visibility into this dynamic learning process.

==> tables/algorithm_classification_threshold.tex <==
\begin{algorithm}
\caption{Classification threshold determination}\label{euclid}

Compute the share of positive tweets per labeled bucket


\textbf{If the first bucket in terms of rank has a share of positives higher than 0.5:}

% \begin{itemize}
$\rightarrow$ Define the \textit{first negative bucket} as the first labeled bucket going down the score distribution with a share of positives lower than 0.5

$\rightarrow$ Compute $r^{*}$ defined as the geometric mean of the mean rank in the bucket preceding the \textit{first negative bucket} in the descending score distribution and the mean rank in the \textit{first negative bucket}
% \end{itemize}

\textbf{Else:}

$\rightarrow$ Set $r^{*}$ to 10, the last rank in the first bucket

Define the classification threshold as the score associated with rank $r^{*}$

\vspace{10mm}

\label{algorithm_classification_threshold}
\end{algorithm}

==> tables/algorithm_classification_threshold_old.tex <==
\begin{algorithm}
\caption{Classification threshold determination}\label{euclid}

Compute the share of positive tweets per labelled bucket


\textbf{If the first bucket in terms of rank has a share of positives higher than 0.5:}

% \begin{itemize}
$\rightarrow$ Define the \textit{first negative bucket} as the first labelled bucket going down the score distribution with a share of positives lower than 0.5

$\rightarrow$ Compute $r^{*}$ defined as the geometric mean of the mean rank in the bucket preceding the \textit{first negative bucket} in the descending score distribution and the mean rank in the \textit{first negative bucket}
% \end{itemize}

\textbf{Else:}

$\rightarrow$ Set $r^{*}$ to 10, the last rank in the first bucket

Define the classification threshold as the score associated with rank $r^{*}$

\vspace{10mm}

\label{algorithm_classification_threshold}
\end{algorithm}

==> tables/archive/table_auc_iter0_2.tex <==
\begin{table*}[!htb]
\centering
\begin{tabular}{|c|c|r|r|r|l|l|}
\hline
\multirow{2}{*}{Country} & \multirow{2}{*}{Model} & \multicolumn{5}{c|}{Class}                                                                                                  \\ \cline{3-7} 
                         &                        & \multicolumn{1}{c|}{Lost Job} & \multicolumn{1}{c|}{Is Hired} & \multicolumn{1}{c|}{Is Unemployed} & Job Offer & Job Search \\ \hline
US                       & Conversational BERT    & 0.959                         & 0.976                         & 0.965                              & 0.985     & 0.98       \\ \hline
Mexico                   & BETO                   & 0.944                         & 0.98                          & 0.949                              & 0.993     & 0.959      \\ \hline
Brazil                   & BERTimbau              & 0.978                         & 0.973                         & 0.949                              & 0.991     & 0.971      \\ \hline

\end{tabular}
\caption{AUROC results on the evaluation set at iteration 0.}
\label{table_auc_iter0}
\end{table*}

==> tables/archive/table_bucket2.tex <==
\begin{table}[hbt!]
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Order of \\ magnitude of\\  the rank\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Number of \\ labelled \\ tweet buckets\end{tabular}} \\ \hline
1                                                                                                           & 5                                                                                       \\ \hline
2                                                                                                           & 2                                                                                       \\ \hline
3                                                                                                           & 3                                                                                       \\ \hline
4                                                                                                           & 4                                                                                       \\ \hline
5                                                                                                           & 5                                                                                       \\ \hline
6                                                                                                           & 1                                                                                       \\ \hline
\end{tabular}
\caption{Number of labelled tweet buckets for each order of magnitude of the rank. The rank is defined as the descending rank in terms of BERT confidence score. Each bucket is made of 10 tweets for a total of 200 labeled tweets.}
\label{tab:sampling_evaluation}
\end{table}

==> tables/archive/table_dataset_description_iter0_2.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Country} & \multirow{2}{*}{Label} & \multicolumn{5}{c|}{Class}                                   \\ \cline{3-7} 
                         &                        & Lost Job & Is Hired & Is Unemployed & Job Offer & Job Search \\ \hline
\multirow{3}{*}{US}      & yes                    & 270      & 334      & 796           & 600       & 524        \\ \cline{2-7} 
                         & no                     & 4239     & 4181     & 3710          & 3918      & 3993       \\ \cline{2-7} 
                         & unsure                 & 15       & 9        & 18            & 6         & 7          \\ \hline
\multirow{3}{*}{Mexico}  & yes                    & 213      & 388      & 1116          & 515       & 659        \\ \cline{2-7} 
                         & no                     & 3488     & 3331     & 2579          & 3210      & 3059       \\ \cline{2-7} 
                         & unsure                 & 28       & 10       & 34            & 4         & 11         \\ \hline
\multirow{3}{*}{Brazil}  & yes                    & 175      & 422      & 925           & 485       & 614        \\ \cline{2-7} 
                         & no                     & 2514     & 2272     & 1761          & 2215      & 2084       \\ \cline{2-7} 
                         & unsure                 & 14       & 9        & 17            & 3         & 5          \\ \hline
\end{tabular}
\caption{Label distribution on the stratified sample for each country and class}
\label{tab:stratified_sample_description}
\end{table*}

==> tables/table_bucket.tex <==
\begin{table}[hbt!]
\centering
\begin{tabular}{l|l}
\toprule
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}l@{}}Order of \\ magnitude of\\  the rank\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Number of \\ labeled \\ tweet buckets\end{tabular}} \\ \midrule
\hfil 1                                                                                                           & \hfil 5                                                                                       \\ \hline
\hfil 2                                                                                                           & \hfil 2                                                                                       \\ \hline
\hfil 3                                                                                                           & \hfil 3                                                                                       \\ \hline
\hfil 4                                                                                                           & \hfil 4                                                                                       \\ \hline
\hfil 5                                                                                                           & \hfil 5                                                                                       \\ \hline
\hfil 6                                                                                                           & \hfil 1                                                                                       \\ \bottomrule
\end{tabular}
\caption{Number of labeled tweet buckets for each order of magnitude of the rank. The rank is defined as the descending rank in terms of BERT confidence score. Each bucket is made of 10 tweets for a total of 200 labeled tweets.}
\label{tab:sampling_evaluation}
\end{table}

==> tables/table_corr_BR_country.tex <==
\begin{table}

\caption{\label{tab:unnamed-chunk-2}Correlation Table: Country-level BR}
\centering
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{1cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c|}{2021 Twitter} & \multicolumn{6}{c}{2020 Twitter} \\
\cline{3-7} \cline{8-13}
  & unrate & is hired 1mo & is unemployed & job offer & job search & lost job 1mo & hire & unemployed & offer & search & loss & out of work\\
\hline
unrate & 1.00 & 0.25 & 0.67 & -0.83 & 0.68 & 0.41 & 0.38 & 0.54 & -0.78 & 0.52 & 0.41 & 0.54\\
\hline
is hired 1mo & 0.25 & 1.00 & 0.82 & -0.32 & 0.75 & 0.73 & 0.78 & 0.57 & 0.22 & 0.66 & 0.56 & 0.68\\
\hline
is unemployed & 0.67 & 0.82 & 1.00 & -0.72 & 0.95 & 0.83 & 0.91 & 0.88 & -0.40 & 0.92 & 0.79 & 0.95\\
\hline
job offer & -0.83 & -0.32 & -0.72 & 1.00 & -0.67 & -0.55 & -0.54 & -0.66 & 0.83 & -0.56 & -0.56 & -0.61\\
\hline
job search & 0.68 & 0.75 & 0.95 & -0.67 & 1.00 & 0.68 & 0.80 & 0.71 & -0.40 & 0.97 & 0.57 & 0.95\\
\hline
lost job 1mo & 0.41 & 0.73 & 0.83 & -0.55 & 0.68 & 1.00 & 0.78 & 0.86 & -0.21 & 0.58 & 0.90 & 0.68\\
\hline
hire & 0.38 & 0.78 & 0.91 & -0.54 & 0.80 & 0.78 & 1.00 & 0.83 & 0.24 & 0.83 & 0.76 & 0.88\\
\hline
unemployed & 0.54 & 0.57 & 0.88 & -0.66 & 0.71 & 0.86 & 0.83 & 1.00 & -0.05 & 0.75 & 0.88 & 0.85\\
\hline
offer & -0.78 & 0.22 & -0.40 & 0.83 & -0.40 & -0.21 & 0.24 & -0.05 & 1.00 & 0.00 & 0.12 & 0.00\\
\hline
search & 0.52 & 0.66 & 0.92 & -0.56 & 0.97 & 0.58 & 0.83 & 0.75 & 0.00 & 1.00 & 0.58 & 0.99\\
\hline
loss & 0.41 & 0.56 & 0.79 & -0.56 & 0.57 & 0.90 & 0.76 & 0.88 & 0.12 & 0.58 & 1.00 & 0.69\\
\hline
out of work & 0.54 & 0.68 & 0.95 & -0.61 & 0.95 & 0.68 & 0.88 & 0.85 & 0.00 & 0.99 & 0.69 & 1.00\\
\hline
\end{tabular}
\end{table}

==> tables/table_corr_CDMX.tex <==
\begin{table}

\caption{\label{tab:unnamed-chunk-2}Correlation Table: City-level Variables CDMX}
\centering
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{1cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c|}{2021 Twitter} & \multicolumn{6}{c}{2020 Twitter} \\
\cline{3-7} \cline{8-13}
  & unrate & is hired 1mo & is unemployed & job offer & job search & lost job 1mo & hire & unemployed & offer & search & loss & out of work\\
\hline
unrate & 1.00 & 0.53 & 0.56 & 0.40 & 0.62 & 0.10 & 0.52 & 0.35 & -0.22 & 0.44 & 0.26 & 0.46\\
\hline
is hired 1mo & 0.53 & 1.00 & 0.86 & 0.68 & 0.93 & 0.32 & 0.86 & 0.28 & -0.14 & 0.80 & 0.13 & 0.68\\
\hline
is unemployed & 0.56 & 0.86 & 1.00 & 0.43 & 0.91 & 0.54 & 0.84 & 0.45 & -0.22 & 0.77 & 0.29 & 0.75\\
\hline
job offer & 0.40 & 0.68 & 0.43 & 1.00 & 0.66 & -0.23 & 0.57 & -0.10 & -0.25 & 0.56 & -0.19 & 0.31\\
\hline
job search & 0.62 & 0.93 & 0.91 & 0.66 & 1.00 & 0.33 & 0.83 & 0.28 & -0.24 & 0.80 & 0.16 & 0.68\\
\hline
lost job 1mo & 0.10 & 0.32 & 0.54 & -0.23 & 0.33 & 1.00 & 0.47 & 0.63 & -0.02 & 0.44 & 0.50 & 0.63\\
\hline
hire & 0.52 & 0.86 & 0.84 & 0.57 & 0.83 & 0.47 & 1.00 & 0.47 & -0.06 & 0.71 & 0.29 & 0.67\\
\hline
unemployed & 0.35 & 0.28 & 0.45 & -0.10 & 0.28 & 0.63 & 0.47 & 1.00 & 0.30 & 0.47 & 0.61 & 0.81\\
\hline
offer & -0.22 & -0.14 & -0.22 & -0.25 & -0.24 & -0.02 & -0.06 & 0.30 & 1.00 & 0.00 & 0.18 & 0.13\\
\hline
search & 0.44 & 0.80 & 0.77 & 0.56 & 0.80 & 0.44 & 0.71 & 0.47 & 0.00 & 1.00 & 0.42 & 0.89\\
\hline
loss & 0.26 & 0.13 & 0.29 & -0.19 & 0.16 & 0.50 & 0.29 & 0.61 & 0.18 & 0.42 & 1.00 & 0.67\\
\hline
out of work & 0.46 & 0.68 & 0.75 & 0.31 & 0.68 & 0.63 & 0.67 & 0.81 & 0.13 & 0.89 & 0.67 & 1.00\\
\hline
\end{tabular}
\end{table}

==> tables/table_corr_MX_country.tex <==
\begin{table}

\caption{\label{tab:unnamed-chunk-2}Correlation Table: Country-level MX}
\centering
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{1cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c|}{2021 Twitter} & \multicolumn{6}{c}{2020 Twitter} \\
\cline{3-7} \cline{8-13}
  & unrate & is hired 1mo & is unemployed & job offer & job search & lost job 1mo & hire & unemployed & offer & search & loss & out of work\\
\hline
unrate & 1.00 & 0.56 & 0.69 & 0.37 & 0.70 & 0.09 & 0.61 & 0.47 & -0.64 & 0.61 & 0.38 & 0.58\\
\hline
is hired 1mo & 0.56 & 1.00 & 0.88 & 0.37 & 0.88 & 0.44 & 0.89 & 0.49 & -0.21 & 0.89 & 0.31 & 0.81\\
\hline
is unemployed & 0.69 & 0.88 & 1.00 & 0.29 & 0.93 & 0.48 & 0.84 & 0.61 & -0.50 & 0.82 & 0.44 & 0.82\\
\hline
job offer & 0.37 & 0.37 & 0.29 & 1.00 & 0.56 & -0.55 & 0.34 & -0.09 & -0.29 & 0.37 & -0.27 & 0.18\\
\hline
job search & 0.70 & 0.88 & 0.93 & 0.56 & 1.00 & 0.20 & 0.82 & 0.44 & -0.50 & 0.83 & 0.23 & 0.74\\
\hline
lost job 1mo & 0.09 & 0.44 & 0.48 & -0.55 & 0.20 & 1.00 & 0.57 & 0.72 & 0.02 & 0.49 & 0.75 & 0.67\\
\hline
hire & 0.61 & 0.89 & 0.84 & 0.34 & 0.82 & 0.57 & 1.00 & 0.72 & -0.39 & 0.89 & 0.62 & 0.88\\
\hline
unemployed & 0.47 & 0.49 & 0.61 & -0.09 & 0.44 & 0.72 & 0.72 & 1.00 & -0.28 & 0.78 & 0.82 & 0.91\\
\hline
offer & -0.64 & -0.21 & -0.50 & -0.29 & -0.50 & 0.02 & -0.39 & -0.28 & 1.00 & -0.34 & -0.20 & -0.34\\
\hline
search & 0.61 & 0.89 & 0.82 & 0.37 & 0.83 & 0.49 & 0.89 & 0.78 & -0.34 & 1.00 & 0.66 & 0.97\\
\hline
loss & 0.38 & 0.31 & 0.44 & -0.27 & 0.23 & 0.75 & 0.62 & 0.82 & -0.20 & 0.66 & 1.00 & 0.79\\
\hline
out of work & 0.58 & 0.81 & 0.82 & 0.18 & 0.74 & 0.67 & 0.88 & 0.91 & -0.34 & 0.97 & 0.79 & 1.00\\
\hline
\end{tabular}
\end{table}

==> tables/table_corr_NYC.tex <==
\begin{table}

\caption{\label{tab:unnamed-chunk-2}Correlation Table: City-level Variables New York}
\centering
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{1cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c|}{2021 Twitter} & \multicolumn{6}{c}{2020 Twitter} \\
\cline{3-7} \cline{8-13}
  & unrate & is hired 1mo & is unemployed & job offer & job search & lost job 1mo & hire & unemployed & offer & search & loss & out of work\\
\hline
unrate & 1.00 & 0.73 & 0.76 & 0.55 & 0.76 & 0.23 & 0.20 & 0.46 & -0.80 & 0.74 & 0.08 & 0.72\\
\hline
is hired 1mo & 0.73 & 1.00 & 0.64 & 0.66 & 0.90 & 0.13 & 0.27 & 0.19 & -0.62 & 0.83 & -0.16 & 0.66\\
\hline
is unemployed & 0.76 & 0.64 & 1.00 & 0.14 & 0.76 & 0.72 & 0.26 & 0.71 & -0.59 & 0.78 & 0.48 & 0.92\\
\hline
job offer & 0.55 & 0.66 & 0.14 & 1.00 & 0.56 & -0.24 & -0.05 & -0.21 & -0.41 & 0.55 & -0.42 & 0.28\\
\hline
job search & 0.76 & 0.90 & 0.76 & 0.56 & 1.00 & 0.25 & 0.31 & 0.29 & -0.63 & 0.93 & -0.07 & 0.79\\
\hline
lost job 1mo & 0.23 & 0.13 & 0.72 & -0.24 & 0.25 & 1.00 & 0.22 & 0.75 & -0.16 & 0.28 & 0.88 & 0.65\\
\hline
hire & 0.20 & 0.27 & 0.26 & -0.05 & 0.31 & 0.22 & 1.00 & 0.10 & -0.14 & 0.43 & 0.16 & 0.44\\
\hline
unemployed & 0.46 & 0.19 & 0.71 & -0.21 & 0.29 & 0.75 & 0.10 & 1.00 & -0.23 & 0.35 & 0.62 & 0.55\\
\hline
offer & -0.80 & -0.62 & -0.59 & -0.41 & -0.63 & -0.16 & -0.14 & -0.23 & 1.00 & -0.68 & -0.04 & -0.64\\
\hline
search & 0.74 & 0.83 & 0.78 & 0.55 & 0.93 & 0.28 & 0.43 & 0.35 & -0.68 & 1.00 & 0.12 & 0.95\\
\hline
loss & 0.08 & -0.16 & 0.48 & -0.42 & -0.07 & 0.88 & 0.16 & 0.62 & -0.04 & 0.12 & 1.00 & 0.40\\
\hline
out of work & 0.72 & 0.66 & 0.92 & 0.28 & 0.79 & 0.65 & 0.44 & 0.55 & -0.64 & 0.95 & 0.40 & 1.00\\
\hline
\end{tabular}
\end{table}

==> tables/table_corr_SP.tex <==
\begin{table}

\caption{\label{tab:unnamed-chunk-2}Correlation Table: City-level Variables São Paulo}
\centering
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{1cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c|}{2021 Twitter} & \multicolumn{6}{c}{2020 Twitter} \\
\cline{3-7} \cline{8-13}
  & unrate & is hired 1mo & is unemployed & job offer & job search & lost job 1mo & hire & unemployed & offer & search & loss & out of work\\
\hline
unrate & 1.00 & -0.11 & 0.51 & -0.82 & 0.44 & 0.17 & 0.34 & 0.49 & -0.12 & 0.51 & 0.31 & 0.57\\
\hline
is hired 1mo & -0.11 & 1.00 & 0.76 & -0.12 & 0.65 & 0.64 & 0.54 & 0.24 & 0.39 & 0.33 & 0.24 & 0.36\\
\hline
is unemployed & 0.51 & 0.76 & 1.00 & -0.62 & 0.89 & 0.78 & 0.78 & 0.66 & -0.01 & 0.77 & 0.48 & 0.84\\
\hline
job offer & -0.82 & -0.12 & -0.62 & 1.00 & -0.49 & -0.44 & -0.48 & -0.57 & 0.39 & -0.48 & -0.41 & -0.57\\
\hline
job search & 0.44 & 0.65 & 0.89 & -0.49 & 1.00 & 0.53 & 0.50 & 0.40 & 0.00 & 0.85 & 0.16 & 0.81\\
\hline
lost job 1mo & 0.17 & 0.64 & 0.78 & -0.44 & 0.53 & 1.00 & 0.76 & 0.62 & -0.04 & 0.38 & 0.67 & 0.52\\
\hline
hire & 0.34 & 0.54 & 0.78 & -0.48 & 0.50 & 0.76 & 1.00 & 0.43 & 0.27 & 0.44 & 0.41 & 0.52\\
\hline
unemployed & 0.49 & 0.24 & 0.66 & -0.57 & 0.40 & 0.62 & 0.43 & 1.00 & 0.05 & 0.40 & 0.42 & 0.65\\
\hline
offer & -0.12 & 0.39 & -0.01 & 0.39 & 0.00 & -0.04 & 0.27 & 0.05 & 1.00 & 0.11 & -0.01 & 0.11\\
\hline
search & 0.51 & 0.33 & 0.77 & -0.48 & 0.85 & 0.38 & 0.44 & 0.40 & 0.11 & 1.00 & 0.08 & 0.95\\
\hline
loss & 0.31 & 0.24 & 0.48 & -0.41 & 0.16 & 0.67 & 0.41 & 0.42 & -0.01 & 0.08 & 1.00 & 0.28\\
\hline
out of work & 0.57 & 0.36 & 0.84 & -0.57 & 0.81 & 0.52 & 0.52 & 0.65 & 0.11 & 0.95 & 0.28 & 1.00\\
\hline
\end{tabular}
\end{table}

==> tables/table_corr_US_country.tex <==
\begin{table}

\caption{\label{tab:unnamed-chunk-2}Correlation Table: Country-level US}
\centering
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{1cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}|>{\raggedleft\arraybackslash}p{0.8cm}}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c|}{2021 Twitter} & \multicolumn{6}{c}{2020 Twitter} \\
\cline{3-7} \cline{8-13}
  & unrate & is hired 1mo & is unemployed & job offer & job search & lost job 1mo & hire & unemployed & offer & search & loss & out of work\\
\hline
unrate & 1.00 & 0.48 & 0.71 & 0.16 & 0.56 & 0.33 & 0.42 & 0.76 & -0.80 & 0.72 & 0.16 & 0.73\\
\hline
is hired 1mo & 0.48 & 1.00 & 0.77 & 0.71 & 0.94 & 0.20 & 0.44 & 0.53 & -0.68 & 0.89 & -0.11 & 0.77\\
\hline
is unemployed & 0.71 & 0.77 & 1.00 & 0.38 & 0.85 & 0.69 & 0.56 & 0.90 & -0.75 & 0.85 & 0.42 & 0.95\\
\hline
job offer & 0.16 & 0.71 & 0.38 & 1.00 & 0.66 & -0.13 & -0.05 & 0.15 & -0.29 & 0.65 & -0.34 & 0.45\\
\hline
job search & 0.56 & 0.94 & 0.85 & 0.66 & 1.00 & 0.28 & 0.52 & 0.64 & -0.77 & 0.96 & -0.04 & 0.86\\
\hline
lost job 1mo & 0.33 & 0.20 & 0.69 & -0.13 & 0.28 & 1.00 & 0.49 & 0.82 & -0.35 & 0.32 & 0.93 & 0.65\\
\hline
hire & 0.42 & 0.44 & 0.56 & -0.05 & 0.52 & 0.49 & 1.00 & 0.70 & -0.50 & 0.67 & 0.35 & 0.73\\
\hline
unemployed & 0.76 & 0.53 & 0.90 & 0.15 & 0.64 & 0.82 & 0.70 & 1.00 & -0.70 & 0.77 & 0.60 & 0.91\\
\hline
offer & -0.80 & -0.68 & -0.75 & -0.29 & -0.77 & -0.35 & -0.50 & -0.70 & 1.00 & -0.77 & -0.11 & -0.76\\
\hline
search & 0.72 & 0.89 & 0.85 & 0.65 & 0.96 & 0.32 & 0.67 & 0.77 & -0.77 & 1.00 & 0.07 & 0.95\\
\hline
loss & 0.16 & -0.11 & 0.42 & -0.34 & -0.04 & 0.93 & 0.35 & 0.60 & -0.11 & 0.07 & 1.00 & 0.38\\
\hline
out of work & 0.73 & 0.77 & 0.95 & 0.45 & 0.86 & 0.65 & 0.73 & 0.91 & -0.76 & 0.95 & 0.38 & 1.00\\
\hline
\end{tabular}
\end{table}

==> tables/table_iterations.tex <==
\begin{table*}
\centering
\label{tab:iterations}
\scalebox{0.63}{
\begin{tabular}{l|l|P{2.1cm}|P{1.8cm}|P{1.9cm}|P{1.9cm}|P{1.9cm}} 
\cmidrule{3-7}
\multicolumn{1}{l}{} &\multicolumn{1}{l}{}  & \textbf{Initial Batch Iteration 0} & \textbf{ConvBERT Iteration 1} & \textbf{ConvBERT Iteration 2} & \textbf{ConvBERT Iteration 3} & \textbf{ConvBERT Iteration 4}  \\ 
\midrule
\multirow{3}{*}{\textbf{Is Unemployed}} & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Lost Job}}      & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Job Search}}    & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Is Hired}}      & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Job Offer}}     & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\
\bottomrule
\end{tabular}
}
\caption{Labeled samples for iteration 0 and iteration 1.}

\end{table*}



% \begin{table*}[ht]
% \caption{Labeled samples for iteration 0 and iteration 1.}
% \label{tab:iterations}
% \centering
% %\begin{minipage}{0.6\textwidth}
% \scalebox{0.63}{
% \begin{tabular}{cc|c|c|c|c|c|}
% \cline{3-7}
% \multicolumn{1}{l}{} & &
% \textbf{\begin{tabular}[c]{@{}c@{}}Initial Batch \\ (iteration 0)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 1)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 4)\end{tabular}} \\ \hline
% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{is\_unemployed}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline
% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{job\_loss}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline

% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{job\_search}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline

% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{is\_hired}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline

% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{job\_offer}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline
% \end{tabular}
% %\end{minipage}
% }
% \end{table*}

==> tables/table_iterations_old.tex <==

\begin{table*}
\centering
\label{tab:iterations}
\scalebox{0.63}{
\begin{tabular}{l|l|P{2.1cm}|P{1.8cm}|P{1.9cm}|P{1.9cm}|P{1.9cm}} 
\cmidrule{3-7}
\multicolumn{1}{l}{} &\multicolumn{1}{l}{}  & \textbf{Initial Batch Iteration 0} & \textbf{ConvBERT Iteration 1} & \textbf{ConvBERT Iteration 2} & \textbf{ConvBERT Iteration 3} & \textbf{ConvBERT Iteration 4}  \\ 
\midrule
\multirow{3}{*}{\textbf{Is Unemployed}} & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Lost Job}}      & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Job Search}}    & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Is Hired}}      & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\ 
\midrule
\multirow{3}{*}{\textbf{Job Offer}}     & positives            & 796                                                      & 818                             & 854                             & 915                             & 960                              \\ 
%\cmidrule{2-7}
                                        & negatives            & 3710                                                     & 4176                            & 4608                            & 5001                            & 5408                             \\ 
%\cmidrule{2-7}
                                        & unsure               & -                                                        & -                               & -                               & -                               & -                                \\
\bottomrule
\end{tabular}
}
\caption{Labeled samples for iteration 0 and iteration 1.}

\end{table*}



% \begin{table*}[ht]
% \caption{Labeled samples for iteration 0 and iteration 1.}
% \label{tab:iterations}
% \centering
% %\begin{minipage}{0.6\textwidth}
% \scalebox{0.63}{
% \begin{tabular}{cc|c|c|c|c|c|}
% \cline{3-7}
% \multicolumn{1}{l}{} & &
% \textbf{\begin{tabular}[c]{@{}c@{}}Initial Batch \\ (iteration 0)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 1)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvBERT\\ (iteration 4)\end{tabular}} \\ \hline
% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{is\_unemployed}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline
% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{job\_loss}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline

% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{job\_search}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline

% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{is\_hired}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline

% \multicolumn{1}{|c|}{} & positives & 796 & 818 & 854 & 915 & 960 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{\textbf{job\_offer}} & negatives & 3710 & 4176 & 4608 & 5001 & 5408 \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & unsure & - & - & - & - & - \\ \hline
% \end{tabular}
% %\end{minipage}
% }
% \end{table*}

==> tables/table_seeds.tex <==
\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
country             & al\_method                                   & iteration & lost\_job\_1mo & is\_hired\_1mo & is\_unemployed & job\_offer & job\_search \\ \hline
\multirow{6}{*}{US} & \multirow{6}{*}{exploit\_explore\_retrieval} & 0         & 14             & 5              & 15             & 10         & 3           \\ \cline{3-8} 
                    &                                              & 1         & 2              & 7              & 2              & 14         & 15          \\ \cline{3-8} 
                    &                                              & 2         & 9              & 1              & 13             & 5          & 6           \\ \cline{3-8} 
                    &                                              & 3         & 11             & 8              & 12             & 2          & 5           \\ \cline{3-8} 
                    &                                              & 4         & 7              & 3              & 4              & 3          & 10          \\ \cline{3-8} 
                    &                                              & 5         & 14             & 11             & 2              & 5          & 10          \\ \hline
\multirow{5}{*}{US} & \multirow{5}{*}{adaptive}                    & 1         & 5              & 5              & 11             & 8          & 8           \\ \cline{3-8} 
                    &                                              & 2         & 14             & 13             & 10             & 2          & 4           \\ \cline{3-8} 
                    &                                              & 3         & 6              & 5              & 5              & 9          & 12          \\ \cline{3-8} 
                    &                                              & 4         & 10             & 2              & 7              & 2          & 12          \\ \cline{3-8} 
                    &                                              & 5         & 6              & 11             & 2              & 9          & 1           \\ \hline
\multirow{5}{*}{US} & \multirow{5}{*}{uncertainty\_calibrated}     & 1         & 11             & 5              & 11             & 10         & 3           \\ \cline{3-8} 
                    &                                              & 2         & 11             & 4              & 2              & 1          & 11          \\ \cline{3-8} 
                    &                                              & 3         & 4              & 2              & 13             & 10         & 1           \\ \cline{3-8} 
                    &                                              & 4         & 1              & 13             & 5              & 9          & 11          \\ \cline{3-8} 
                    &                                              & 5         & 2              & 3              & 9              & 5          & 4           \\ \hline
\multirow{5}{*}{US} & \multirow{5}{*}{uncertainty\_uncalibrated}   & 1         & 4              & 7              & 12             & 1          & 13          \\ \cline{3-8} 
                    &                                              & 2         & 10             & 14             & 1              & 11         & 1           \\ \cline{3-8} 
                    &                                              & 3         & 5              & 1              & 8              & 14         & 8           \\ \cline{3-8} 
                    &                                              & 4         & 2              & 12             & 12             & 3          & 11          \\ \cline{3-8} 
                    &                                              & 5         & 12             & 9              & 1              & 4          & 13          \\ \hline
\multirow{6}{*}{BR} & \multirow{6}{*}{exploit\_explore\_retrieval} & 0         & 12             & 5              & 5              & 6          & 8           \\ \cline{3-8} 
                    &                                              & 1         & 6              & 6              & 10             & 8          & 4           \\ \cline{3-8} 
                    &                                              & 2         & 10             & 7              & 11             & 9          & 8           \\ \cline{3-8} 
                    &                                              & 3         & 6              & 1              & 6              & 12         & 1           \\ \cline{3-8} 
                    &                                              & 4         & 6              & 1              & 2              & 2          & 1           \\ \cline{3-8} 
                    &                                              & 5         & 13             & 11             & 4              & 6          & 5           \\ \hline
\multirow{6}{*}{MX} & \multirow{6}{*}{exploit\_explore\_retrieval} & 0         & 10             & 8              & 12             & 2          & 1           \\ \cline{3-8} 
                    &                                              & 1         & 8              & 6              & 2              & 7          & 6           \\ \cline{3-8} 
                    &                                              & 2         & 14             & 15             & 12             & 10         & 2           \\ \cline{3-8} 
                    &                                              & 3         & 2              & 9              & 10             & 10         & 8           \\ \cline{3-8} 
                    &                                              & 4         & 4              & 9              & 9              & 3          & 1           \\ \cline{3-8} 
                    &                                              & 5         & 2              & 3              & 6              & 5          & 7           \\ \hline
\end{tabular}
\end{table*}

==> tables/table_seeds_old.tex <==
\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
country             & al\_method                                   & iteration & lost\_job\_1mo & is\_hired\_1mo & is\_unemployed & job\_offer & job\_search \\ \hline
\multirow{6}{*}{US} & \multirow{6}{*}{exploit\_explore\_retrieval} & 0         & 14             & 5              & 15             & 10         & 3           \\ \cline{3-8} 
                    &                                              & 1         & 2              & 7              & 2              & 14         & 15          \\ \cline{3-8} 
                    &                                              & 2         & 9              & 1              & 13             & 5          & 6           \\ \cline{3-8} 
                    &                                              & 3         & 11             & 8              & 12             & 2          & 5           \\ \cline{3-8} 
                    &                                              & 4         & 7              & 3              & 4              & 3          & 10          \\ \cline{3-8} 
                    &                                              & 5         & 14             & 11             & 2              & 5          & 10          \\ \hline
\multirow{5}{*}{US} & \multirow{5}{*}{adaptive}                    & 1         & 5              & 5              & 11             & 8          & 8           \\ \cline{3-8} 
                    &                                              & 2         & 14             & 13             & 10             & 2          & 4           \\ \cline{3-8} 
                    &                                              & 3         & 6              & 5              & 5              & 9          & 12          \\ \cline{3-8} 
                    &                                              & 4         & 10             & 2              & 7              & 2          & 12          \\ \cline{3-8} 
                    &                                              & 5         & 6              & 11             & 2              & 9          & 1           \\ \hline
\multirow{5}{*}{US} & \multirow{5}{*}{uncertainty\_calibrated}     & 1         & 11             & 5              & 11             & 10         & 3           \\ \cline{3-8} 
                    &                                              & 2         & 11             & 4              & 2              & 1          & 11          \\ \cline{3-8} 
                    &                                              & 3         & 4              & 2              & 13             & 10         & 1           \\ \cline{3-8} 
                    &                                              & 4         & 1              & 13             & 5              & 9          & 11          \\ \cline{3-8} 
                    &                                              & 5         & 2              & 3              & 9              & 5          & 4           \\ \hline
\multirow{5}{*}{US} & \multirow{5}{*}{uncertainty\_uncalibrated}   & 1         & 4              & 7              & 12             & 1          & 13          \\ \cline{3-8} 
                    &                                              & 2         & 10             & 14             & 1              & 11         & 1           \\ \cline{3-8} 
                    &                                              & 3         & 5              & 1              & 8              & 14         & 8           \\ \cline{3-8} 
                    &                                              & 4         & 2              & 12             & 12             & 3          & 11          \\ \cline{3-8} 
                    &                                              & 5         & 12             & 9              & 1              & 4          & 13          \\ \hline
\multirow{6}{*}{BR} & \multirow{6}{*}{exploit\_explore\_retrieval} & 0         & 12             & 5              & 5              & 6          & 8           \\ \cline{3-8} 
                    &                                              & 1         & 6              & 6              & 10             & 8          & 4           \\ \cline{3-8} 
                    &                                              & 2         & 10             & 7              & 11             & 9          & 8           \\ \cline{3-8} 
                    &                                              & 3         & 6              & 1              & 6              & 12         & 1           \\ \cline{3-8} 
                    &                                              & 4         & 6              & 1              & 2              & 2          & 1           \\ \cline{3-8} 
                    &                                              & 5         & 13             & 11             & 4              & 6          & 5           \\ \hline
\multirow{6}{*}{MX} & \multirow{6}{*}{exploit\_explore\_retrieval} & 0         & 10             & 8              & 12             & 2          & 1           \\ \cline{3-8} 
                    &                                              & 1         & 8              & 6              & 2              & 7          & 6           \\ \cline{3-8} 
                    &                                              & 2         & 14             & 15             & 12             & 10         & 2           \\ \cline{3-8} 
                    &                                              & 3         & 2              & 9              & 10             & 10         & 8           \\ \cline{3-8} 
                    &                                              & 4         & 4              & 9              & 9              & 3          & 1           \\ \cline{3-8} 
                    &                                              & 5         & 2              & 3              & 6              & 5          & 7           \\ \hline
\end{tabular}
\end{table*}
